Making Large Language Models Better Knowledge Miners for Online Marketing with Progressive Prompting Augmentation

Nowadays, the rapid development of mobile economy has promoted the flourishing of online marketing campaigns, whose success greatly hinges on the efficient matching between user preferences and desired marketing campaigns where a well-established Marketing-oriented Knowledge Graph (dubbed as MoKG) could serve as the critical "bridge" for preference propagation. In this paper, we seek to carefully prompt a Large Language Model (LLM) with domain-level knowledge as a better marketing-oriented knowledge miner for marketing-oriented knowledge graph construction, which is however non-trivial, suffering from several inevitable issues in real-world marketing scenarios, i.e., uncontrollable relation generation of LLMs,insufficient prompting ability of a single prompt, the unaffordable deployment cost of LLMs. To this end, we propose PAIR, a novel Progressive prompting Augmented mIning fRamework for harvesting marketing-oriented knowledge graph with LLMs. In particular, we reduce the pure relation generation to an LLM based adaptive relation filtering process through the knowledge-empowered prompting technique. Next, we steer LLMs for entity expansion with progressive prompting augmentation,followed by a reliable aggregation with comprehensive consideration of both self-consistency and semantic relatedness. In terms of online serving, we specialize in a small and white-box PAIR (i.e.,LightPAIR),which is fine-tuned with a high-quality corpus provided by a strong teacher-LLM. Extensive experiments and practical applications in audience targeting verify the effectiveness of the proposed (Light)PAIR.

==> code.tex <==
\clearpage
\appendix
\section{Code}
\begin{algorithm}[t]
\small
\caption{PEACE}
\begin{algorithmic}[1]
\Require $\mathcal{H}^\mathcal{S},\mathcal{H}^\mathcal{T},\mathcal{N}{(e, r)}$.
\Ensure Pretrained model, user interest-specific representation
set $\{\bm{z}_u^{\mathcal{A}}\}$, entity representation set $\{\bm{h}_e\}$.
\LeftComment  \textbf{\textit{Pre-training Stage}}
\State Initialize prototype  $\mathbf{P}$
\While{\textit{not converged}}
\State Calculate entity representation $\bm{h}_e$ (Eqn \ref{eq:he}).
\State Calculate user interest-specific representation
set $\bm{z}_u^{\mathcal{A}}$ (Eqn \ref{eq:domain-specific}). 

\State Calculate similarity vector $\mathbf{S}_e$ between $\bm{h}_e$ and $\mathbf{P}$ (Eqn \ref{eq:sim}).
\State Generate the prototype-level view of entity $\hat{\bm{h}}_e$ (Eqn \ref{eq:pt_view} ).
\State Estimate contrastive prototype learning loss $\mathcal{L}_{\mathcal{CP}}$ (Eqn \ref{eq:loss_cp}).
\State Calculate K-largest mask vector $\bm{m}_i$ (Eqn \ref{eq:mask}).   
\State Calculate user scenario-aware representation $\hat{\bm{z}}_u^{\mathcal{A}}$ (Eqn \ref{eq:hatz}).
\State Calculate user universal encoding $\bm{z}_u$ (Eqn \ref{eq:universal}).
\State Estimate entity-oriented pre-training loss $\mathcal{L}_{\mathcal{ET}}$ (Eqn \ref{eq:loss_et}).
\State Minimize loss in source domain $\mathcal{L}_{\mathcal{PT}}$ (Eqn \ref{eq:loss_source}).
 
\LeftComment  \textbf{\textit{Off-line Inference}}
\State Caculate $\{\bm{z}_u^{\mathcal{A}}\}$ and save it to \textbf{Embedding Storage}.
\State Caculate $\{\bm{h}_e\}$ and save it to \textbf{Embedding Storage}. 

\LeftComment  \textbf{\textit{Fine-tuning Stage}}
\State Restore parameters from the pretrained model.
\State Load user representation $\bm{z}_u^{\mathcal{T}}$ from \textbf{Embedding Storage}.
\State Caculate item representation $\bm{z}_i^{\mathcal{T}}$ by mean pooling of associated entities retrieved from \textbf{Embedding Storage}. 
\While{\textit{not converged}}
\State Caculate preference score $\hat{y}_{ui}$ (Eqn \ref{eq:y_target}).
\State Minimize loss in target domain $\mathcal{L}_{\mathcal{FT}}$ (Eqn \ref{eq:loss_target}).

\end{algorithmic}
\label{alg:peace_psuedo}
\end{algorithm}









==> tab/application.tex <==
% \begin{table*}[t]\centering
% \setlength{\tabcolsep}{1.2mm}
% {

% \caption{The performance of user targeting application with {\kg}.} 
% \label{tab:application}
% \begin{tabular}{c|c|c|c}

% \toprule
%  {Domain}& {Before}
%  & {After} 
% & {Improvement}   \\ 
% % \cline{4-11}
% %\midrule
% \cmidrule{1-4}
% %\midrule
% {} & {} 
%  & {} & {}  \\ 
% \midrule
% {} & {} 
%  & {} & {}  \\ 
% \midrule
% {} & {} 
%  & {} & {}  \\ 
% \midrule

% {} & {} 
%  & {} & {}  \\ 

% \bottomrule
% \end{tabular}
% }
% \end{table*}









==> tab/prompt.tex <==
% \onecolumn
\begin{table*}[t]
\setlength{\tabcolsep}{0.6mm}
\setlength\lightrulewidth{0.8pt}
\setlength\heavyrulewidth{0.3ex}
\caption{An example (source entity: Uncle Fruit, relation: related product) of calling an LLM to carry out progressive prompting augmentation, where different types of knowledge is distinguished by color, \ie \textcolor{blue}{Struc\_KG},  \textcolor{red}{Desc\_KG} and  \textcolor{green}{Inher\_KG}.}
\label{tab:uncle_fruit_examples}
  \centering
    \begin{tabular}{ll}
      \toprule 
      {\textbf{Augmented Prompt 1} } & {Please list at least 8 related products of the \textcolor{blue}{brand "Uncle Fruit"}, separated by commas, and output the result} \\
      {\textbf{}} & {in the following format: Related product: [\textcolor{green}{fruit}, , ,]. } \\
     \midrule
      {\textbf{Output 1} } & {Related product: [fruit, dried fruit, jam, fruit vinegar, fruit juice, fruit and vegetable juice,nuts, fruit tea].} \\
     \midrule
    {\textbf{Augmented Prompt 2}} & {Please list at least 8 related products of the \textcolor{blue}{brand "Uncle Fruit"}, separated by commas, and output the result} \\
      {\textbf{}} & {in the following format: Related product: [\textcolor{blue}{fruit sales, fruit, grocery shopping, fresh produce}, , , ]. } \\
     \midrule
      {\textbf{Output 2} } & {Related product: [fruit sales, fruit, grocery shopping, fresh produce, fruit delivery service,  fruit gift boxes, } \\
      {\textbf{}} & {fruit juice drinks, fruit delivery].} \\
     \midrule
      {\textbf{Augmented Prompt 3}} & {\textcolor{red}{Some keywords related to the brand "Uncle Fruit" are: fruit sales, fruit, grocery shopping, and fresh produce.} } \\
      {} & {Please list at least 8 related products of the \textcolor{blue}{brand "Uncle Fruit"}, separated by commas, and output the result } \\
      {} & {in the following format: Related product: [\textcolor{green}{fruit}, , , ].} \\
     \midrule
      {\textbf{Output 3} } & {Related product: [fruit, vegetables, nuts, dried fruit, fresh meal packs, fruit gift boxes, fruit platters, fruit ice } \\
      {\textbf{}} & {cream].  } \\
     \midrule
      {\textbf{Augmented Prompt 4}} & {\textcolor{red}{Some keywords related to the brand "Uncle Fruit" are: fruit sales, fruit, grocery shopping, and fresh produce.} } \\
      {} & {Please list at least 8 related products of the \textcolor{blue}{brand} \textcolor{blue}{"Uncle Fruit"}, separated by commas,  and output the result  } \\
      {\textbf{}} & {in the following format: Related product: [\textcolor{blue}{fruit sales, fruit, grocery shopping, fresh produce}, , , ].} \\
     \midrule
      {\textbf{Output 4} } & {Related product: [fruit sales, fruit, grocery shopping, fresh produce, fruit platters, fruit and vegetable delivery, } \\
      {\textbf{}} & {fresh fruit juice, fruit gift boxes].} \\
     \midrule
      {\textbf{Augmented Prompt 5}} & {\textcolor{red}{Some keywords related to the brand "Uncle Fruit" are: fruit sales, fruit, grocery shopping, and fresh produce.} } \\
      {} & {Please list at least 8 related products of the \textcolor{blue}{brand}  \textcolor{blue}{"Uncle Fruit"}, separated by commas,  and output the result} \\
      {\textbf{}} & {in the following format: Related product: [, , , ].} \\
     \midrule
      {\textbf{Output 5} } & {Related product: [fruit sales, fruit gift boxes, fruit platters, fresh vegetables,  seafood, poultry and eggs, dairy } \\
      {\textbf{}} & {and beverages, snacks].} \\
     \midrule
     \midrule
      {\textbf{Non-augmented Prompt} } & {Please list at least 8 related products of "Uncle Fruit", separated by commas,  and output the result in the } \\
      {\textbf{} } & {following format: Related product: [, , ,]. } \\
     \midrule
      % \hline
      {\textbf{Output} } & {Related product: [Uncle Fruit watch, Uncle Fruit earphones, Uncle Fruit smart  bracelet, Uncle Fruit power } \\
      {\textbf{}} & {bank, Uncle Fruit selfie stick, Uncle Fruit data cable,  Uncle Fruit insulated cup, Uncle Fruit electric skateboard]. } \\
    \bottomrule
\end{tabular}
\end{table*}


\begin{table*}[t]
\setlength{\tabcolsep}{0.6mm}
\setlength\lightrulewidth{0.8pt}
\setlength\heavyrulewidth{0.3ex}
\caption{An example (source entity: CKA, relation: related organization) of calling an LLM to carry out progressive prompting augmentation.}
  \centering
    \begin{tabular}{ll}
      \toprule 
      % \hline
      {\textbf{Augmented Prompt 1} } & {Please list at least 8 related organizations of the \textcolor{blue}{event "CKA"}, separated by commas, and output the result in } \\
      {} & {the following format: Related organization: [\textcolor{green}{China Wushu Sanda Super League Organizing Committee}, , ,]. } \\
      % {} & { } \\
     \midrule
      % \hline
      {\textbf{Output 1}} & {Related organization: [China Wushu Sanda Super League Organizing Committee,  Chinese Sanda Association, } \\
      {} & {World Sanda Federation, Chinese Wushu Research Institute,  General Administration of Sport of China Wushu } \\
      {} & {Sports Management Center, Asian Sanda Federation, Chinese Wushu Association, Chinese Wushu Artists } \\
      {} & {Association].  } \\
     \midrule
      % \hline
    {\textbf{Augmented Prompt 2} } & {\textcolor{red}{Information related to the event "CKA" includes: Gene granule cell therapy CKA, Chinese Karate Association }  } \\
    {} & {\textcolor{red}{CKA, China Wushu Sanda Super League. From 1960, when Bruce Lee brought Chinese Kung Fu to the world, } } \\
    {} & {\textcolor{red}{to 1994 when Jackie Chan successfully entered Hollywood, Chinese Kung Fu has become the best window for } } \\
    % {} & { \textcolor{red}{} } \\
    {} & { \textcolor{red}{China to showcase its 5000-year culture to the world.} Please list  at least 8 related organizations of the \textcolor{blue}{event}} \\
    {} & {\textcolor{blue}{ "CKA"}, separated by commas, and output the result in the following format: Related organization: [ \textcolor{green}{China }} \\
    % {} & {} \\
      {} & {\textcolor{green}{Wushu Sanda Super League Organizing Committee}, , , ]. } \\
     \midrule
      % \hline
      {\textbf{Output 2}} & {Related organization: [Gene Granule Cell Therapy Research Institute, Chinese Karate Association, China } \\
      {} & {Wushu Sanda Super League Organizing Committee, Chinese Wushu Association, Chinese Wushu Artists } \\
      {} & {Association, Chinese Kung Fu Association, General Administration of Sport of China Wushu Sports } \\
      {} & {Management Center, Beijing Wushu Association].} \\
      % {} & {} \\
     \midrule
      % \hline
       {\textbf{Augmented Prompt 2} } & {\textcolor{red}{Information related to the event "CKA" includes: Gene granule cell therapy CKA, Chinese Karate Association }  } \\
    {} & {\textcolor{red}{CKA, China Wushu Sanda Super League. From 1960, when Bruce Lee brought Chinese Kung Fu to the world, } } \\
    {} & {\textcolor{red}{to 1994 when Jackie Chan successfully entered Hollywood, Chinese Kung Fu has become the best window for } } \\
    % {} & { \textcolor{red}{} } \\
    {} & { \textcolor{red}{China to showcase its 5000-year culture to the world.} Please list  at least 8 related organizations of the \textcolor{blue}{event}} \\
    {} & {\textcolor{blue}{event "CKA"} , separated by commas, and output the result in the following format: Related organization: [, , , ]. } \\
    % {} & {} \\
     \midrule
      % \hline
      { \textbf{Output 3}} & {Related organization: [Chinese Karate Association, China Wushu Sanda Super League, General Administration } \\
      {} & {of Sport of China Wushu Sports Management Center, Chinese Wushu Association, Chinese Karate Union,  } \\
      % {} & {} \\
      {} & {World Wildlife Fund, National Martial Arts Grading Examination Committee,International Wushu Federation].} \\
     \midrule
     \midrule
      {\textbf{Non-augmented Prompt}} & {Please list at least 8 related organizations of "CKA", separated by commas,   and output the result in the following} \\
      { } & {format: Related organization: [, , ,]. } \\
     \midrule
      % \hline
      {\textbf{LLM Output} } & {Related organization: [Linux Foundation, CNCF, Red Hat, IBM, Kubernetes official, CoreOS, Tencent Cloud, } \\
      {} & {Alibaba Cloud]. } \\
    \bottomrule
    % \hline
    
\end{tabular}
\label{tab:CKA_examples}
%\vspace{-10pt}
\end{table*}

\begin{table*}[t]
% \small
\setlength{\tabcolsep}{0.6mm}
\setlength\lightrulewidth{0.8pt}
\setlength\heavyrulewidth{0.3ex}
\caption{An example (source entity: air, relation: related brand) of calling an LLM to carry out progressive prompting augmentation.}
  \centering
    \begin{tabular}{ll}
      \toprule 
      % \hline
      {\textbf{Augmented Prompt 1}} & {Please list at least 8 related brands of the \textcolor{blue}{product "air"}, separated by commas, and   output the result in the } \\
      {} & {following format: Related brand: [\textcolor{green}{Puma, Adidas, Nike}, , , , ]. } \\
     \midrule
      % \hline
      {\textbf{Output 1} } & {Related brand: [Air Jordan, Airwalk, Air Max, Air Force 1, Airtech, Airwalk, Airbourne, Air Step]. } \\
      % {} & {} \\
     \midrule
      % \hline
    {\textbf{Augmented Prompt 2}} & {Please list at least 8 related brands of the \textcolor{blue}{product "air"} , separated by commas, and   output the result in the} \\
      {} & {following format: Related brand: [\textcolor{blue}{footwear}, , , ].} \\
     \midrule
      % \hline
       % {} & { } \\
      {\textbf{Output 2}} & {Related brand: [Nike, Adidas, Puma, Reebok, Converse, Under Armour, Vans,  New Balance].} \\
      % {} & {} \\
     \midrule
      % \hline
      {\textbf{Augmented Prompt 3}} & {\textcolor{red}{A keyword related to the product "air" is: footwear.} Please list at least 8 related brands   of the \textcolor{blue}{product "air"}, } \\
      {} & {separated by commas, and output the result in the following format: Related brand: [\textcolor{green}{Puma, Adidas, Nike}, , , , ]. } \\
     \midrule
      {\textbf{Output 3}} & {Related brand: [Nike, Jordan, Airwalk,Reebok, Skechers, New Balance, Fila, Converse].} \\
     \midrule
      {\textbf{Augmented Prompt 4}} & {\textcolor{red}{A keyword related to the product "air" is: footwear.} Please list at least 8 related brands of the \textcolor{blue}{product "air"}, } \\
      {} & {separated by commas, and output the result in the   following format: Related brand: [\textcolor{blue}{footwear}, , , ].} \\
      % {} & {} \\
     \midrule
      {\textbf{Output 4}} & {Related brand: [Nike, Adidas, Jordan, Puma, New Balance, Converse, Reebok, Vans]. } \\
      % {} & {} \\
     \midrule
      {\textbf{Augmented Prompt 5}} & {\textcolor{red}{A keyword related to the product "air" is: footwear.} Please list at least 8 related brands of the \textcolor{blue}{product "air"}, } \\
      {} & {separated by commas, and output the result in the  following format: Related brand: [, , , ].} \\
      % {} & {} \\
     \midrule
      {\textbf{Output 5}} & {Related brand: [Nike, Jordan, Adidas, Puma, Reebok, Converse, New Balance, ASICS]. } \\
      % {} & {} \\
     \midrule
     \midrule
      {\textbf{Non-augmented Prompt}} & {Please list at least 8 related brands of the product "Air", separated by commas,   and output the result in the } \\
      { } & {following format: Related brand: [,,,].} \\
     \midrule
      {\textbf{Output}} & {Related brand: [Air Jordan, AirPods, Air Max, Air Force 1, Air Wick, Air France, AirAsia, Air Canada].} \\
      % {} & {} \\
    \bottomrule
\end{tabular}
\label{tab:air_examples}
%\vspace{-10pt}
\end{table*}
